Enhancing ASIC Technology Mapping via Parallel Supergate Computing

With the development of large-scale integrated circuits, electronic design automation~(EDA) tools are increasingly emphasizing efficiency, with parallel algorithms becoming a trend. The optimization of delay reduction is a crucial factor for ASIC technology mapping, and supergate technology proves to be an effective method for achieving this in EDA tools flow. However, we have observed that increasing the number of generated supergates can reduce delay, but this comes at the cost of an exponential increase in computation time. In this paper, we propose a parallel supergate computing method that addresses the tradeoff between time-consuming and delay optimization. The proposed method utilizes the input-constrained supergate pattern to parallelly generate the supergate candidates, and then filter the valid supergates as the results. Experiment results show the efficiency of the proposed method, for example, it can attain the improvement of 4x speedup in computation time and 10.1 in delay reduction with 32 threads.

==> sections/0-abstract.tex <==
\begin{abstract}

% Technology mapping is an essential step in EDA flow. 
% However, the function of the circuit may be changed after technology mapping, and equivalence checking (EC) based verification is highly necessary. 
% The traditional EC method has significant time and resource constraints, making it only feasible to carry out at a coarse-grained level. 
% To make it efficient for technology mapping, we propose a fine-grained method called MEC, which leverages a combination of two approaches to significantly reduce the time cost of verification. 
% The local block verification approach performs fast verification and the global graph cover approach guarantees correctness. 
% The proposed method is rigorously tested and compared to three EC tools, and the results show that MEC technique offers a substantial improvement in speed. 
% MEC not only offers a faster and more efficient way of performing EC on technology mapping but also opens up new opportunities for more fine-grained verification in the future.

\end{abstract}


\begin{IEEEkeywords}

% Technology mapping, equivalence checking, Fine-grained, FPGA

\end{IEEEkeywords}

==> sections/1-introduction.tex <==
\section{Introduction}

Technology mapping is a crucial step in the logic synthesis of Electronic Design Automation (EDA) flow for digital systems, such as ASICs and FPGAs. 
It involves converting a technology-independent logical network into a  functionally equivalent circuit implemented using primitive gates selected from a technology library. 
The primary objective is to minimise some objectives such as area subject to certain constraints such as delay\cite{chatterjee2007algorithms}.

The process of ASIC technology mapping involves the translation of the logic network into a predefined set of standard cells. 
In recent developments, there has been a shift in ASIC technology mapping from tree-based mapping \cite{tree-mapping} to cut-based mapping \cite{priority-cut}. 
Cut-based methods offer enhanced exploration of diverse logic structures and optimization, particularly with scalability to large-scale designs.
The limited standard cells in the standard cell library can not meet all the cut functions, which makes some possibilities lost in the mapping process.
The emergence of supergates technology enables the standard cell library to display more structural composite gates to achieve more functions to meet the needs of mapping and to achieve a lower delay.

The increasing complexity of SoC design and the market pressure to reduce time to market, make the systems designer's task harder especially for ASIC design\cite{ASIC-time}.
However, technology mapping becomes time-consuming due to the booming scale and complexity of IC designs\cite{ASIC-time2}. 
Because of the high computational complexity of supergate, using this technology when mapping will even increase the time by hundreds of times, so it is rarely used in the actual mapping process.
parallel works

\todo{show supergate' value}

Our contributions can be divided into three parts:
\begin{itemize}
    \item We 
    \item We 
    \item We 
\end{itemize}

The rest of this paper is organized as follows:
Section II provides background information on ASIC technology mapping and supergate.
Section III 
Section IV  shows the framework of our work.
Section V  presents the results of our experiments on equivalence checking during technology mapping.
Finally, the conclusion and future work are summarized in Section VI.


==> sections/2-preliminaries.tex <==
\section{Preliminaries}

In this section, we consider the ASIC technology mapping. 
And we will introduce some of the basics we might need later.

\textbf{Boolean function.}
An n-variable Boolean function f(x) takes the form f: $\{0, 1\}^{n}$ → {0, 1}, where \{0, 1\} is the Boolean domain and n is the arity of f.
Boolean function $f$ is often represented by its truth table T($f$), a string of $2^{n}$ bits. 
In the process of ASIC mapping, the functions of standard cells are represented through the truth table. 
For example, the AND2 gate has a 16-bit truth table of 0001 0001 0001 0001.


\textbf{And-Inverter Graph (AIG).} Traditional ASIC technology mapping algorithm is based on Boolean Network AIG(And-Inverter Graph). 
An AIG is a DAG(directed acyclic graph) which is a typical representation of the logical functionality of a circuit. 
In AIG, nodes are implemented using AND2 gates, and edges represent inverted or non-inverted signals. The \textit{primary inputs}~(PIs) are nodes without fanins.

\textbf{ $k$-feasible Cut.} The cut $C$ of a node $v$ is a set of nodes such that every path from primary inputs (PIs) to $v$ must pass through at least one node of cut $C$.
A \textit{trivial cut} of node $v$ is the node itself. 
A \textit{non-trivial cut} includes all the nodes that are found on the paths from the root to the leaves.
A cut is $k$-\textit{feasible} if the number of nodes in it does not exceed $k$.
The local function of the cut $C$ can be calculated by assigning the truth table of elementary variables to its leaf node and then simulated bit operation. 
The calculated truth table of the root node $v$ is the local function of the cut $C$.


\textbf{Cut enumeration.}
The cut enumeration incrementally calculates the cut set(k-feasible cuts) for each node from the bottom up of PIs. Given two cut sets, $CS_1$ and $CS_2$, the merge operation of the cut sets, $CS_1 \diamond CS_2$, is defined as:
$$
CS_1 \diamond CS_2 = \{u \cup v | u \in CS_1, v \in CS_2\}
\eqno{(1)}
$$

Let $\Phi(n)$ be the set of $k$-feasible cuts for node $n$, $n_1$ and $n_2$ denote to $n$'s fanins.
The set of cuts of node $n$ is computed using sets of cuts of its fanins:  

$$
\Phi(n) = \left\{
\begin{aligned}
\{\{n\}\} & :n\in PIs \\
\{\{n\}\} \cup \Phi(n_1) \diamond \Phi(n_2)  & :otherwise
\end{aligned}
\right \}.
\eqno{(2)}
$$

\begin{example}

As shown in Fig.~\ref{fig:prelim-cut-enum}, The calculation process of the cut set is consistent with the above equations.
Note that, the cut\{1, 2, 3, 4, 5\} is not a 4-feasible cut which contains 5 nodes, and needs to be dropped.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/cut_enum.PNG}
    \caption{An AIG and cut enumeration.}
    \label{fig:prelim-cut-enum}
\end{figure}

\end{example}


\textbf{Supergate.} A supergate is a single-output combinational network of a small number of library gates. 
As shown in Fig. \ref{fig:prelim-supergate}, it is a supergate composed of an AND gate, an OR gate, and a NOT gate. 
In the ASIC technology mapping process, if a cut's function cannot be found in the standard cell library, it will be discarded, even if it would be a better choice. 
In summary, supergate can implement more functional combinations of gates in the gates library, allowing for more cuts during the mapping process that can be found in the library.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/supergate.PNG}
    \caption{A supergate composed of an AND gate, an OR gate and a NOT gate.}
    \label{fig:prelim-supergate}
\end{figure}

\begin{example}

The cut \{3, 4, 5\} of node 8 in Fig. \ref{fig:prelim-cut-enum} has a function of (3 + !5) * (4 + !5), which is simplified to 3 * 4 + !5. 
It can directly use the supergate in Fig. \ref{fig:prelim-supergate} for cover. 
However, if there are only three basic gates in the standard cell library, the cover result of cut \{3, 4, 5\} will not occur.
\todo{variables should use domain variables notation}

\end{example}


\textbf{Boolean matching.}

An NP transformation of a Boolean function involves variable negations and permutations. 
Negation replaces a variable with its complement (e.g., x1 → !x1). 
Permutation changes the order of variables (e.g., x1x2 → x2x1). 
For an n-variable Boolean function, there are $2^{n}$ ways of transformations by flipping the inputs and n! ways of transformations by swapping the variables. 
Additionally, there are two polarities of the function derived by complementing its output. 
In total, there are $2^{n+1}n!$ transformations of the function by swapping its inputs and flipping its inputs and output.

==> sections/3-techmap.tex <==
\section{Analysis and Motivation}

In this section, we will outline the basic flow for ASIC technology mapping and supergate, then, we will analyze the supergate and introduce the motivation behind this work.

\subsection{ASIC technology mapping}

Fig. \ref{fig:techmap-flow} depicts the traditional ASIC technology mapping flow.  
In the following subsections, we will briefly introduce the process of the ASIC mapping algorithm. \\

\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/mapping.png}
    \caption{ASIC mapping flow.}
    \label{fig:techmap-flow}
\end{figure}

\subsubsection{Generate Library}
\ \newline 
\indent For library generation, the purpose is to generate a hash table indexed to the corresponding functional standard cells list through the truth table, which is used in subsequent Boolean matching stages.
For gates extracted from the library file, the first step is to calculate their truth table based on their functional expressions. 
The area and input/output port information can be directly extracted, and the pin delay needs to be estimated using the load-independent model.
For the extracted gates, as shown in Fig. \ref{fig:prelim-permute}, using different input permutations to generate different truth tables to expand the standard cell library.
Finally, each gate should calculate the N-canonical of the truth table and add it to the list with this as the key in the hash table. N-canonical is the lexicographically small truth table in its $N$ class, called $n$ representative Two functions are in the same N class if one can obtain one from the other by input negations

The process of generating a supergate candidate is shown in Fig. \ref{fig:prelim-supergate}. First, select a standard gate from the library as the root gate, use the existing supergates as the fanins, and enumerate its potential combinations to create higher-level supergate candidates.
Note that the set of super variables that can be used at first is the set of elementary variables, and their number is usually no more than the  \todo{max size of cut input.}
\todo{write an Algorithm for supergate computing}


Recursively go through the above steps to generate higher-level supergate candidates. 
Before adding a new supergate candidate to the hash table, need to compare whether it is the best delay and area among the candidates with the same function. The best can be retained, and the worst needs to be deleted.

Finally, we need to select the candidates who have the correct function to be effective supergates. The correct function requires that all its elementary variables are continuous. For example, NAND2 ($a$, $c$) or NAND2 (b, c) needs to be screened out, while NAND2 (a, b) can be left.

\subsubsection{Mapping}
\ \newline 
\indent For boolean matching, the purpose is to calculate the gates library corresponding to each cut of each node, which is the match of that cut.
To calculate the match corresponding to a cut, it is necessary to first calculate the local function of the cut, which is represented by a truth table. 

Then, the N-canonical of the truth table is used to index gates in the library.
In this way, a set of gates with the same function as the cut and an opposite set of gates will be obtained. 
The opposite gates can realize their function by adding an inverter to the output.
Sometimes the delay of an inverter plus an AND2 gate is smaller than that of a NAND2 gate, so this method can increase flexibility and make the mapping result better.

Depth-oriented mapping sorts the cuts of each node, using the delay implemented by the corresponding match of the cut as the basis for sorting. 
The representative cut is the one that can achieve the minimum delay.
In the subsequent area recovery stage, it is essentially sorting the cuts, and then performing a secondary sorting through heuristic area calculation in the cuts obtained from the depth-oriented mapping of the optimal delay, to optimise the area without increasing the delay.
After completing the steps above, we can obtain the mapping result by traversing the network in reverse topological order and gathering the representative cuts of the utilized nodes.
Finally, map the cut to its corresponding match, which is the specific implementation of the gate, to convert AIG into a gate-level netlist.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/permute.PNG}
    \caption{Different input permutations generate different truth tables.}
    \label{fig:prelim-permute}
\end{figure}


\subsection{Complexity of Supergate Computing}

Supergates can significantly optimize the delay of AIG. 
Although it will increase a certain area, the reduction of delay is more valuable. However, ABC only implements this function but does not explicitly give the command to use supergates.
It can only be opened by modifying the code, and the default time limit is 100 seconds for the whole calculation process.
This has something to do with the time-consuming computation of supergates.
The calculation process and complexity can be seen from the following formula:

\begin{equation}
\text{sg}(l) = 
\left\{
\begin{aligned}
k && \quad (\text{level} = 1) \\
\sum_{g=1}^{G} \sum_{i=1}^{\text{inputs\_num}(g)} P(\text{sg}(l-1), i) && \quad (\text{level} = l) 
\end{aligned}
\right.
\end{equation}

The calculation of supergates is a recursive process. 
When the $level$ is $1$, the number of supergates is equal to the maximum number of inputs $k$ of the gates supported by the library. 
When the $level$ is $l$, the calculation process is to traverse the root gates set $G$ and select the fanin gates from the supergate set at level l-1.
The range of $i$ is 1 to $inputs\_num(g)$, the number of inputs of root gate $g$, and there are different fanin gates permutations.
\todo{Supergate solution Space Complexity}


\begin{example}

It can be seen from the formula that its computational complexity is high. 
For a group of only 100 different standard cells with 4 inputs, theoretically, it can generate as many as 4,074,775 supergate candidates with only level 2.
In ASIC technology mapping using supergates, computing supergates will occupy most of the time of the whole process, and the memory required is huge.

\end{example}

==> sections/4-method.tex <==
\section{ASIC technology mapping with parallel supergates computing }

In this section, we will first analyze the traditional ASIC technology mapping with supergates, and then introduce our parallel supergates computing framework.

As shown in algorithm \ref{algorithm:method-flow}, the flow of our parallel supergates computing can be roughly divided into the following four parts: (1) Pre-processing; (2) Parallel compute candidates; (3) Parallel filter supergates; (4) ASIC technology mapping; The fourth part refers to some additional operations that need to be done in the ASIC technology mapping part.

\begin{algorithm}
\small
\caption{Parallel Supergates Computing Flow}
\label{algorithm:method-flow}
\begin{algorithmic}[1]
\Require Library $L$, inputs size $k$, max level $ml$, threads num $N$

\Statex /* init candidates storage $C$ and hash table $H$ */ 
\State $C$, $H$ $\leftarrow$ init\_data\_structure($N$)

\Statex /* Filter available root gates from library $L$ */ 
\State $roots$ $\leftarrow$ collect\_root\_gates($L$, $k$)

\Statex /* Create initial supergates as elementary variables  */ 
\State $C$ $\leftarrow$ create\_first\_supergates($k$)

\Statex /* Parallel compute supergate candidates in level $l$  */ 
\For {$l$++ $<$ $ml$}
    \State $C$ $\leftarrow$ parallel\_compute\_candidates($roots$, $k$, $C$, $H$, $N$)
\EndFor

\Statex /* Parallel filter correct supergates from candidates */
\State $L$ $\leftarrow$ parallel\_driven\_supergates($H$, $N$)
\end{algorithmic}
\end{algorithm}

\subsection{pre-processing}
Some preprocessing work needs to be done before the computing of supergates candidates is officially started. 
First, we need to explain the design of the supergates storage model and hash table, as well as the initialisation of the hash table.

The supergate candidates include also valid patterns and invalid ones, but we need to save them instead of filtering them out the first time, because they may still be useful.
\todo{valid, invalid}\\
\todo{please add some definitions about Boolean variable value continous }\\
\todo{please add some definitions about supergate \& subsupergate}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/pattern_combine.png}
    \caption{invalid patterns combine to a valid supergate.}
    \label{fig:method-combine}
\end{figure}

\begin{example}

As shown in Fig. \ref{fig:method-combine}, an AND2 gate with the wrong function comprises initial variables $x1$ and $x3$. 
Assuming that the truth table is 16 bits, TT ($x1$)=0101 0101 0101 0101, 
\todo{all possible value of x1}
TT ($x3$)=0000 1111 0000 1111, the result of the bit-parallel simulation of the two is 0000 0101 0000 0101, which is not a correct truth table of AND2 gate.
However, in the computing of supergates at the next level, this AND2 gate and an OR2 gate are combined to form a supergate of three consecutive initial variable inputs, and the truth table of this supergate will be correct.
Therefore, all calculated supergate candidates will be stored.

\end{example}

To support the multi-threaded storage of candidates, there are several storage queues for threads, and each thread has a queue to avoid conflicts.

The hash table to be used in the next stage is mapped from the truth table to the pointer list of the corresponding candidates. 
Since the candidates generated by multiple threads may have the same truth table in a multithreaded environment, it is necessary to use mutex locks to avoid conflicts.
The range of truth tables is very large. The range of the truth table of 5 variables is $2^{32}$.
To save time and space, map the truth table to a smaller range of keys, and then initialise the corresponding number of mutexes.

Finally, the gates that can be used as roots are selected from the standard cells, and $k$ supergates representing elementary variables are generated.
The gates of the same function in the standard cells will only leave the one that has the lowest delay.

\subsection{parallel compute candidates}

The following is the main body of the Parallel Compute Candidates algorithm for computing the superrates of each level.

\begin{algorithm}
\small
\caption{Parallel Compute Candidates}
\label{algorithm:method-parallel-compute}
\begin{algorithmic}[1]
\Require candidates set $C$, hash table $H$, root gates $roots$, inputs size $k$, prune limit $limit$, threads num $N$

\Statex /* collect fanin gates candidates in $C$, which are smallest delay in same function */ 

\State $F$ $\leftarrow$ collect\_fanin\_gates\_candidates($C$)

\ForAll{$r \in \text{parallel range}(1, |roots|, N)$}

\If{$r$.inputs\_num $>$ $limit$ }:
   \State \textbf{continue}
\EndIf

\Statex /* collect fanin gates candidates for root $r$ */ 
\State $f$ $\leftarrow$ collect\_fanin\_gates($F$, $r$)

\Statex /* recursive enumerate fanins permutations */ 
\State $fa \gets \text{new array}[k]$
\State $idx \gets \text{0}$
\State recur\_enum\_perm($C$, $H$, $r$, $f$, $fa$, $idx$)

\EndFor

\end{algorithmic}
\end{algorithm}

Algorithm \ref{algorithm:method-parallel-compute} first selects the gate with the smallest delay among the supergate candidates of the same function in $C$ as the candidates of fanins gates. 
All roots that meet the input limit are processed in parallel. 
First, collect fanin gates candidates that adapt to the current root $r$, and then use a recursive algorithm to enumerate all combinations between them.

\begin{algorithm}
    \caption{Recursive Enumerate Combinations}
    \label{algorithm:method-recursive}
    \begin{algorithmic}[1]
        \Require candidates set $C$, hash table $H$, root gates $roots$, fanins gates $fanins$, fanins array $fa$, index in fanins array $idx$
        
        \If{$fn == r.inputs\_num$}:
            \State $a$, $d$, $f \leftarrow compute\_composed\_data(r, fa)$
            \If{is\_best($a$, $d$, $f$)}:
                \State $C, H \leftarrow create\_new\_candidate(r, fa, a, d, f)$
            \EndIf
        \Else
            \For{$f$ in $fa$}
                \If{!is\_repetitive()}:
                    \State $fa$[$idx$] $\leftarrow$ $f$
                    \State recur\_enum\_perm($C, H, r, fanins, fa, idx$)
                \EndIf
            \EndFor
        \EndIf
    \end{algorithmic}
\end{algorithm}

Algorithm \ref{algorithm:method-recursive} is a method based on backtracking and recursion, which is used to enumerate all combinations of a root gate and several fanins gates.
The $fanins$ is all available fanins gates.
The current fanin gates combination is stored in $fa$, and $idx$ is the position in the fanins array to be modified.

Before a new supergate candidate is created, need to calculate its area, delay and truth table, and then compare whether it is the smallest delay in the same function in the hash table.
Note that there may be multiple optimal supergate candidates for the same function, and all of them need to be preserved.
The successfully created supergate candidate is stored in the queue exclusive to each thread, and their pointers are added to the hash table.
Here, the operation of the hash table needs to obtain the corresponding mutex to avoid conflict.

\subsection{parallel filter supergates}

After generating all the supergate candidates, need to filter out the part with the correct function, which is the final supergates.
Since the storage mode of supergate candidates is queue storage with several threads, the filtering steps can also be carried out in parallel.
However, in the end, it is necessary to add the pointer of valid supergate candidates to the library, and the library is also a truth table indexed to the hash table of corresponding supergates, so it is also necessary to re-hash and mutex lock to avoid multi-threaded write conflicts.


\subsection{asic mapping}

Because parallel supergates computing can generate a lot of supergates, the number of indexes in each truth table will also be very large. 
To balance efficiency and quality, it is necessary to limit the number of overrides attempted by each cut in the depth-oriented mapping and area recovery stages. 
This can sacrifice a small part of the quality in exchange for a huge speed increase.

==> sections/5-experiments.tex <==
\section{Experiment}

\subsection{Setup}
\textbf{Environment.} 
We implemented the proposed method using GCC 11.1.0 x86 version on a 64-bit Ubuntu 18.04.6 system. 
We collected our experimental results on a system with 128G shared RAM and 2 Intel® Xeon® Gold 6252 CPU @ 2.10GHz processors, each with 48 physical cores.

\textbf{Benchmarks.}
We perform experiments on EPFL benchmark\cite{benchmark}. 
This benchmark contains 10 arithmetic circuits and 10 control/random circuits with circuit sizes ranging from 0.1k to 210k.
The library is sky130\_fd\_sc\_hd\_\_tt\_025C\_1v80, which contains 82 useful gates for supergates computing.

\textbf{Parameters.}
For the parameters of supergates computing, the maximum input number of the library is 5, and the level of supergates is 2.
For ASIC technology mapping, the cut enumeration limit is 24, and each cut tries 30 supergates.

\subsection{Result}

To demonstrate the scalability of parallel supergates computing, we present in Fig. \ref{fig:experiment-speedup} and Fig. \ref{fig:experiment-num} the comparison of the number and time of supergates generated by our method with ABC under different threads, the speedup is our method run time divide the runtime of ABC supergates computing, which is 100s.
The above results were performed 20 times under each thread, and the average was taken for display to eliminate external noise effects.

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/speedup.PNG}
    \caption{rum time in different threads number compare with ABC.}
    \label{fig:experiment-speedup}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/supergates-num.PNG}
    \caption{generated supergates number in different threads number compare with ABC.}
    \label{fig:experiment-num}
\end{figure}

From Figures \ref{fig:experiment-speedup} and \ref{fig:experiment-num} above, it can be seen that the supergate computing time of ABC was fixed at 100 seconds, resulting in 6050082 supergates being generated. 
And our method can generate 6710591 supergates in 115.38 seconds when the number of threads is 1, with a speed similar to ABC.
However, our method can generate more supergates when the number of threads is higher, and the number of supergates generated may vary in a multi-threaded environment.

\begin{table*}[htb]
	\centering
	\caption{QoR.}
	\renewcommand\tabcolsep{9.4pt}
	\label{table: QoR}
	\begin{tabular}{|c|rrr|rrr|rr|}
		\hline
		\multirow{2}{*}{Benchmark name} & \multicolumn{3}{c|}{without supergates} & \multicolumn{3}{c|}{with supergates(32 thr)} & \multicolumn{2}{c|}{QoR improve(\text{\%})}                                                                                                                                         \\ \cline{2-9}
		                                & \multicolumn{1}{r|}{Area}               & {delay}                                      & {time}                           & \multicolumn{1}{r|}{Area}      & {delay}                         & \multicolumn{1}{r|}{time}  & \multicolumn{1}{r|}{area}   & {delay} \\ \hline
		priority                        & \multicolumn{1}{r|}{4390.46}            & \multicolumn{1}{r|}{15308.35}                & \multicolumn{1}{r|}{0.08}        & \multicolumn{1}{r|}{7525.97}   & \multicolumn{1}{r|}{11072.87}   & \multicolumn{1}{r|}{0.2}   & \multicolumn{1}{r|}{-71.42} & 27.67   \\
		cavlc                           & \multicolumn{1}{r|}{2158.32}            & \multicolumn{1}{r|}{1432.44}                 & \multicolumn{1}{r|}{0.07}        & \multicolumn{1}{r|}{2289.7}    & \multicolumn{1}{r|}{1591.95}    & \multicolumn{1}{r|}{0.1}   & \multicolumn{1}{r|}{-6.09}  & -11.14  \\
		arbiter                         & \multicolumn{1}{r|}{39051.2}            & \multicolumn{1}{r|}{6956.59}                 & \multicolumn{1}{r|}{14.88}       & \multicolumn{1}{r|}{50593.52}  & \multicolumn{1}{r|}{5721.77}    & \multicolumn{1}{r|}{7.07}  & \multicolumn{1}{r|}{-29.56} & 17.75   \\
		i2c                             & \multicolumn{1}{r|}{4579.39}            & \multicolumn{1}{r|}{1812.74}                 & \multicolumn{1}{r|}{0.16}        & \multicolumn{1}{r|}{4598.16}   & \multicolumn{1}{r|}{1375.52}    & \multicolumn{1}{r|}{0.13}  & \multicolumn{1}{r|}{-0.41}  & 24.12   \\
		voter                           & \multicolumn{1}{r|}{62513.7}            & \multicolumn{1}{r|}{5521.48}                 & \multicolumn{1}{r|}{3.54}        & \multicolumn{1}{r|}{67236.98}  & \multicolumn{1}{r|}{6063.34}    & \multicolumn{1}{r|}{6.07}  & \multicolumn{1}{r|}{-7.56}  & -9.81   \\
		int2float                       & \multicolumn{1}{r|}{741.96}             & \multicolumn{1}{r|}{988.29}                  & \multicolumn{1}{r|}{0.02}        & \multicolumn{1}{r|}{787}       & \multicolumn{1}{r|}{865.55}     & \multicolumn{1}{r|}{0.03}  & \multicolumn{1}{r|}{-6.07}  & 12.42   \\
		ctrl                            & \multicolumn{1}{r|}{471.7}              & \multicolumn{1}{r|}{618.92}                  & \multicolumn{1}{r|}{0.01}        & \multicolumn{1}{r|}{482.96}    & \multicolumn{1}{r|}{661.38}     & \multicolumn{1}{r|}{0.02}  & \multicolumn{1}{r|}{-2.39}  & -6.86   \\
		dec                             & \multicolumn{1}{r|}{1186.14}            & \multicolumn{1}{r|}{635.01}                  & \multicolumn{1}{r|}{0.11}        & \multicolumn{1}{r|}{1186.14}   & \multicolumn{1}{r|}{635.01}     & \multicolumn{1}{r|}{0.04}  & \multicolumn{1}{r|}{0.00}   & 0.00    \\
		mem\_ctrl                       & \multicolumn{1}{r|}{147591.55}          & \multicolumn{1}{r|}{18593.08}                & \multicolumn{1}{r|}{7.85}        & \multicolumn{1}{r|}{151561.61} & \multicolumn{1}{r|}{16666.21}   & \multicolumn{1}{r|}{13.04} & \multicolumn{1}{r|}{-2.69}  & 10.36   \\
		router                          & \multicolumn{1}{r|}{982.19}             & \multicolumn{1}{r|}{3139.95}                 & \multicolumn{1}{r|}{0.05}        & \multicolumn{1}{r|}{1013.47}   & \multicolumn{1}{r|}{2439.37}    & \multicolumn{1}{r|}{0.04}  & \multicolumn{1}{r|}{-3.18}  & 22.31   \\ \hline
		log2                            & \multicolumn{1}{r|}{102559.61}          & \multicolumn{1}{r|}{35324.38}                & \multicolumn{1}{r|}{7.09}        & \multicolumn{1}{r|}{108769.31} & \multicolumn{1}{r|}{35862}      & \multicolumn{1}{r|}{8.48}  & \multicolumn{1}{r|}{-6.05}  & -1.52   \\
		square                          & \multicolumn{1}{r|}{64865.96}           & \multicolumn{1}{r|}{17519.39}                & \multicolumn{1}{r|}{1.89}        & \multicolumn{1}{r|}{64785.88}  & \multicolumn{1}{r|}{14709.86}   & \multicolumn{1}{r|}{3.45}  & \multicolumn{1}{r|}{0.12}   & 16.04   \\
		adder                           & \multicolumn{1}{r|}{5228.76}            & \multicolumn{1}{r|}{13858.53}                & \multicolumn{1}{r|}{0.02}        & \multicolumn{1}{r|}{4979.78}   & \multicolumn{1}{r|}{13804.78}   & \multicolumn{1}{r|}{0.08}  & \multicolumn{1}{r|}{4.76}   & 0.39    \\
		sin                             & \multicolumn{1}{r|}{20313.23}           & \multicolumn{1}{r|}{17250.48}                & \multicolumn{1}{r|}{1.20}        & \multicolumn{1}{r|}{21276.66}  & \multicolumn{1}{r|}{16219.6}    & \multicolumn{1}{r|}{1.39}  & \multicolumn{1}{r|}{-4.74}  & 5.98    \\
		div                             & \multicolumn{1}{r|}{227212.91}          & \multicolumn{1}{r|}{430705.56}               & \multicolumn{1}{r|}{5.62}        & \multicolumn{1}{r|}{249187.73} & \multicolumn{1}{r|}{315822.66}  & \multicolumn{1}{r|}{12.04} & \multicolumn{1}{r|}{-9.67}  & 26.67   \\
		hyp                             & \multicolumn{1}{r|}{885183.94}          & \multicolumn{1}{r|}{3856567.75}              & \multicolumn{1}{r|}{22.86}       & \multicolumn{1}{r|}{889927.25} & \multicolumn{1}{r|}{2114426.25} & \multicolumn{1}{r|}{49.51} & \multicolumn{1}{r|}{-0.54}  & 45.17   \\
		max                             & \multicolumn{1}{r|}{11193.24}           & \multicolumn{1}{r|}{21940.98}                & \multicolumn{1}{r|}{4.11}        & \multicolumn{1}{r|}{11831.35}  & \multicolumn{1}{r|}{18415.66}   & \multicolumn{1}{r|}{1.88}  & \multicolumn{1}{r|}{-5.70}  & 16.07   \\
		sqrt                            & \multicolumn{1}{r|}{98034.02}           & \multicolumn{1}{r|}{935573.5}                & \multicolumn{1}{r|}{3.43}        & \multicolumn{1}{r|}{143128.52} & \multicolumn{1}{r|}{1148640.75} & \multicolumn{1}{r|}{5.43}  & \multicolumn{1}{r|}{-46.00} & -22.77  \\
		multiplier                      & \multicolumn{1}{r|}{93659.83}           & \multicolumn{1}{r|}{23105.71}                & \multicolumn{1}{r|}{ 3.48}       & \multicolumn{1}{r|}{95352.7}   & \multicolumn{1}{r|}{19142.62}   & \multicolumn{1}{r|}{5.88}  & \multicolumn{1}{r|}{-1.81}  & 17.15   \\
		bar                             & \multicolumn{1}{r|}{10896.7}            & \multicolumn{1}{r|}{4816.15}                 & \multicolumn{1}{r|}{0.35}        & \multicolumn{1}{r|}{10896.7}   & \multicolumn{1}{r|}{4816.15}    & \multicolumn{1}{r|}{0.51}  & \multicolumn{1}{r|}{0.00}   & 0.00    \\ \hline
		\textbf{Average}                & \multicolumn{1}{r|}{}                   & \multicolumn{1}{r|}{}                        & \multicolumn{1}{r|}{}            & \multicolumn{1}{r|}{}          & \multicolumn{1}{r|}{}           & \multicolumn{1}{r|}{}      & \multicolumn{1}{r|}{-9.95}  & 9.50    \\ \hline
	\end{tabular}
\end{table*}

To demonstrate the optimization effect of our method on subsequent mapping, we present the mapping results of our method at 32 threads and without using supergate in Table \ref{table: QoR}. 
For the output netlist, we use \textit{stime} command of ABC to calculate its area and delay.

From the table \ref{table: QoR}, it can be seen that after using parallel supergate, with a thread count of 32, the area increases by 9.95\text{\%}, the delay decreases by 9.5\text{\%}, and the time increases by no more than 2 times compared to not using supergate.

\todo{show the comparison of valid cuts between with/W.o supergate}

==> sections/6-conclusion.tex <==
\section{Conclusion}

In this work, we propose a parallel supergates computing algorithm for ASIC technology mapping.
We analyze the complexity and effectiveness of supergates computing and propose the value of parallel computing.
We designed the framework of parallel supergates computing and the corresponding organization of shared data structure so that supergates computing can be carried out in parallel.
The combination of recursion and backtracking is used to enumerate supergates, which effectively avoids the storage of intermediate variables and saves space.
Finally, we also compared the speed of generating supergates with ABC and also showed the optimization effect of supergates on mapping results.
